Blocks Assemble! Learning to Assemble with Large-Scale Structured Reinforcement Learning

Assembly of multi-part physical structures is both a valuable end product for autonomous robotics, as well as a valuable diagnostic task for open-ended training of embodied intelligent agents. We introduce a naturalistic physics-based environment with a set of connectable magnet blocks inspired by children's toy kits. The objective is to assemble blocks into a succession of target blueprints. Despite the simplicity of this objective, the compositional nature of building diverse blueprints from a set of blocks leads to an explosion of complexity in structures that agents encounter. Furthermore, assembly stresses agents' multi-step planning, physical reasoning, and bimanual coordination. We find that the combination of large-scale reinforcement learning and graph-based policies -- surprisingly without any additional complexity -- is an effective recipe for training agents that not only generalize to complex unseen blueprints in a zero-shot manner, but even operate in a reset-free setting without being trained to do so. Through extensive experiments, we highlight the importance of large-scale training, structured representations, contributions of multi-task vs. single-task learning, as well as the effects of curriculums, and discuss qualitative behaviors of trained agents.

==> background.tex <==
\section{Background}

==> ethics.tex <==
\section{Broader Impact Statement}
    Ethics Statement
    \begin{itemize}
        \item Once robotics assembly is solved, it will have significant economic impacts, many of which can be negative such as job displacement, etc.
        \item When developing such systems in production, we must carefully study how they can be introduced in society in a manner that minimizes the potential for harm
    \end{itemize}
    
    Climate Impact
    \begin{itemize}
        \item Large scale compute is needed to do rollouts. Developments such as Brax~\cite{freeman2021brax} and Nvidia Isaac Gym~\cite{makoviychuk2021isaac} which enable running thousands of environments in parallel using limited hardware will massively reduce the climate footprint of training such models.
    \end{itemize}

